How Auditing Methodologies Can Impact Our Understanding of YouTube's Recommendation Systems

Data generated by audits of social media websites have formed the basis of our understanding of the biases presented in algorithmic content recommendation systems. As legislators around the world are beginning to consider regulating the algorithmic systems that drive online platforms, it is critical to ensure the correctness of these inferred biases. However, as we will show in this paper, doing so is a challenging task for a variety of reasons related to the complexity of configuration parameters associated with the audits that gather data from a specific platform. Focusing specifically on YouTube, we show that conducting audits to make inferences about YouTube's recommendation systems is more methodologically challenging than one might expect. There are many methodological decisions that need to be considered in order to obtain scientifically valid results, and each of these decisions incur costs. For example, should an auditor use (expensive to obtain) logged-in YouTube accounts while gathering recommendations from the algorithm to obtain more accurate inferences? We explore the impact of this and many other decisions and make some startling discoveries about the methodological choices that impact YouTube's recommendations. Taken all together, our research suggests auditing configuration compromises that YouTube auditors and researchers can use to reduce audit overhead, both economically and computationally, without sacrificing accuracy of their inferences. Similarly, we also identify several configuration parameters that have a significant impact on the accuracy of measured inferences and should be carefully considered.

==> tables/channel-table.tex <==
\begin{table*}
	\centering
	\begin{tabular}{c c c c c}
    \toprule
& Mean$_{1}$ & Mean$_{2}$ & T-test & Significant \\
    \hline

	login & 0.541893 & 0.544320 & 0.991694 & N\\
	login niche & 1.338929 & 1.155815 & 0.445847 & N\\
	login mainstream & 1.010998 & 0.929439 & 0.725158 & N\\
	login maintrain & 0.905653 & 1.451738 & 0.027024 & Y\\
	history & 0.406826 & 0.759438 & 0.118794 & N\\
	10vs25 & 0.112398 & 0.096477 & 0.839969 & N\\
	50vs100 & 0.174907 & 0.285266 & 0.484881 & N\\
	get click & 0.186560 & 0.236107 & 0.735900 & N\\
		

    \hline
	\end{tabular}
	\captionsetup{width=.60\textwidth}
    \caption{Statistical significance test results for channel entropies.}
    \label{tab:channel-table}
\end{table*}


==> tables/content-table.tex <==
\begin{table*}
\centering
\begin{tabular}{c c c c c} 
\toprule
& Mean$_{1}$ & Mean$_{2}$ & T-test & Significant\\
\hline


login & 0.049383 & 0.049293 & 0.993650 & N\\
login niche & 0.056579 & 0.048934 & 0.591882 & N\\
login mainstream & 0.050185 & 0.048007 & 0.848398 & N\\
login maintrain & 0.053478 & 0.051956 & 0.905021 & N\\
history & 0.046980 & 0.047497 & 0.962153 & N\\
10vs25 & 0.035124 & 0.034968 & 0.985361 & N\\
25vs50 & 0.040292 & 0.039026 & 0.890621 & N\\
50vs100 & 0.037104 & 0.038047 & 0.918071 & N\\
no login & 0.045668 & 0.046199 & 0.960421 & N\\
get click & 0.039285 & 0.036522 & 0.763649 & N\\

\hline
\end{tabular}
\captionsetup{width=.60\textwidth}
\caption{Statistical significance test results for tree content.}
\label{tab:content-table}
\end{table*}


==> tables/result-means.tex <==
\begin{table*}
	\centering
	\begin{tabular}{c c c}
    \toprule
    & \multicolumn{2}{c}{\textbf{Means}} \\
    & Content 
    & Views \\ 
    \hline

    $S_{NM}(R_{C},T)$ & 0.0930 & 8405329 \\
    $S_{NN}(R_{C},T)$ & 0.1102 & 3916774 \\
    $S_{MM}(R_{C},T)$ & - & -  \\
    $S_{MN}(R_{C},T)$ & - & -  \\

    \hline
	\end{tabular}
	\captionsetup{width=.60\textwidth}
    \caption{Statistical significance test results, $S$ denotes the similarity
    between the training-set $T$ and the recommendations $R_{C}$, with the subscripts denoting the combinations of niche/mainstream
    training-sets and seeds.}
    \label{tab:result-means}
\end{table*}


==> tables/result-stats.tex <==
\begin{table*}
	\centering
	\begin{tabular}{c cc  cc  cc}
    \toprule
    & \multicolumn{2}{c}{\textbf{Content}} & \multicolumn{2}{c}{\textbf{Views}} & \multicolumn{2}{c}{\textbf{Channels}}\\
    & Difference 
    & SS
    & Difference 
    & SS 
    & Difference
    & SS \\
    \hline
    
    $S_{NM}(R_{C},T)$ vs $S_{NN}(R_{C},T)$ & -0.0172 & T & 4488555 & T &  -0.7043 & T \\
    % 0.0323 & 1.269e-17  & 2.596 & 6.541 \\
    $S_{MM}(R_{C},T)$ vs $S_{MN}(R_{C},T)$ & -0.0079 & F & 7732025 & T &  -0.2085 & F \\
    
    \hline
	\end{tabular}
	\captionsetup{width=.60\textwidth}
    \caption{Statistical significance test results, $S$ denotes the similarity
    between the training-set $T$ and the recommendations $R_{C}$, with the subscripts denoting the combinations of niche/mainstream
    training-sets and seeds. Channels$_1$ and Channels$_2$ denote the channel distributions of each of the crawls.}
    \label{tab:result-stats}
\end{table*}


==> tables/results.tex <==
\begin{table*}
	\centering
	\begin{tabular}{c  c c  c c}
    \toprule
    & \multicolumn{2}{c}{\textbf{T-test}} & \multicolumn{2}{c}{\textbf{Entropy}} \\
    & Content 
    & Views 
    & Channels$_{1}$ 
    & Channels$_{2}$ \\
    \hline
    
    $S_{NM}(R_{C},T)$ vs $S_{NN}(R_{C},T)$ & 0.019 & 0.001  & 2.596 & 6.541 \\
    $S_{MM}(R_{C},T)$ vs $S_{MN}(R_{C},T)$ & - & - & - & - \\
    
    \hline
	\end{tabular}
	\captionsetup{width=.60\textwidth}
    \caption{Statistical significance test results, $S$ denotes the similarity
    between the training-set $T$ and the recommendations $R_{C}$, with the subscripts denoting the combinations of niche/mainstream
    training-sets and seeds. Channels$_1$ and Channels$_2$ denote the channel distributions of each of the crawls.} 
    \label{tab:results}
\end{table*}


==> tables/train-set-means.tex <==
\begin{table}[t]
\small
	\centering
	\begin{tabular}{c c c c c}
	\toprule
	& Abortion Rights & Climate Change & Flat Earth & Feminism \\
	\midrule

		Mainstream & 2.66 & 11.08 & 3.68 & 6.41 \\
		Niche      & 0.01  & 0.04 & 0.02 & 0.03 \\


	\midrule
	\end{tabular}
	\caption{Mean (in millions) number of views for the traning sets used. 
	\blue{Replace Feminism with Women Rights. This table goes to appendix}}
	\label{tab:train-means}
\end{table}



==> tex-files/results.tex <==
\section{Results} \label{sec:results}


\subsection{Seed selection}



We first analyze the impact the seed has on the recommendations. We evaluate training-set like trees with each other, varying only the seed
and then evaluating the differences in the observed recommendations. If the seed has a significant impact in terms of swaying the 
recommendations, despite a training-set consisting on $n$-videos, we can conclude that researchers must account for this 
impact in terms of any testable hypothesss. Tables \ref{tab:result-stats} and \ref{tab:result-means} show the results of the seed-bias tests. 
We conclude the following:


\input{tables/result-stats.tex}

\input{tables/content-table.tex}

\input{tables/channel-table.tex}

\input{tables/views-table.tex}


\subsubsection{Seed selection has an impact on the content seen.} In order to show this, need to prove that there is a statistically
significant difference, in terms of content, when the seed is varied despite keeping constant training-set.

\parai{Methodology.}We leverage LDA to extract the topics of the trees, by path, and compute 
the cosine-similarity scores of the path topics and the training-set topics. We then ascertain the statistical significance of this
difference by running a T-test \cite{ttest} between the cosine-similarity of the training-sets and the recommendations. If the seed
does not impact the recommendations, we would not observe a statistically significant difference between the recommendation trees
generated using the varying seeds.

\parai{Evaluation.}Trees with the like training-sets but varying niche/mainstream seeds see different content when compared to the respective training-sets. We see that the recommendations are \emph{more similar} to the training-set when the seed picked is consistent
with the niche/mainstream appeal of the training set. We also see that the $p$-values of the difference in cosine-similarity scores is 
less than a significance-level of $0.05$. This result has a direct impact on bias research, as simply switching seeds with differing
mainstream appeal will significantly impact the quality of the content observed in the recommendations, despite a watch-history with completely
different content in comparsion to the seed. Researchers $A$ and $B$, both running independent measurements to study the impact the recommendation system has on the resulting content, will conclude different content biases,
simply because the seed picked by $A$ and $B$ did not belong to the same niche/mainstream group, despite using the same watch-histories.

\input{tables/result-means.tex}

\subsubsection{Seed selection has an impact on recommended videos' popularity.} In order to show that the recommendation popularity is biased by seed selection,
we need to show that across like training-sets, varying the seed results in statistically significant difference in the views of the resulting recommendation. 

\parai{Methodology.}We compare the two trees with different seeds by (1) calculating the mean views of each tree, and (2) run a T-test between the views of the
two trees.

\parai{Evaluation.}There is statistically significant difference in the resulting views as a result of varying the seed, with a $p$-value $<0.05$, with the means
of the two trees differing by over two-times. Simply changing the seed and keeping all other factors constant results in twice as many views in the recommendations. This suggests that measurements aiming to prove a popularity bias on YouTube must factor in the impact of selecting a seed that may naturally be
geared towards more popular content in comparsion to niche content. 

\subsubsection{Seed selection has an impact on the resulting channel diversity.} In order to show that recommendation channel diversity has a direct correlation 
with the seed selection, we must show that the number of channels seen, as well as he relative frequency of 
these channels vary significantly based on the seed. 

\parai{Methodology.}We calculate the entropy of each of the trees, which gives us a measure of the uncertainity
of getting a channel given a particular seed. A higher value of entropy would mean that there is a higher number of channels in that particular tree, with frequency distributions such that probability of picking channel A over 
channel B is higher in this tree when compared to the other tree.

\parai{Evaluation.}Trees with like training-sets and varying seeds result in a \emph{significantly} high 
difference in entropy between the channel distributions of the two trees. Table \ref{tab:result-stats} shows that 
the entropy nearly \emph{triples} if the seed changes from a mainstream to a niche seed. Manual inspection showed
that the majority of the channels in the mainstream-seed tree were the channel of the seed. The implication of this is that any 
inference made in terms of the channel distribution disparity is contingent on the seed picked for any bias measurement. 
Researcher A opting for a niche seed for their measurement would conclude that the recommendation system has a 
divergent bias, whereas reseacher B opting for a mainstream seed would conclude that the recommendation system has a converging bias, highlighting the need for increased scrunity in seed selection.  


\subsection{Profile type}
\subsubsection{The type of profile used impacts the recommendations trees.} 

% \subsubsection{The positive/negative user-level signals impact the recommendations seen.}

\subsection{Watch-times and histories}
\subsubsection{Clearing user watch histories results in a fresh profile state.}

% \subsection{Inference testing framework} \label{sec:inferences}

% \subsubsection{What metrics are used to evaluate the differences between recommendation trees?} \label{metrics} In order to evaluate the differences between the observed recommendations,
% we must extract the content in these videos and map them to a relative scale. Based on where the videos lie on that scale, we evaluate the recommendation tree divergence based on the levels. 
% The exact metrics themselves are hypothesis dependent, as the type of content studied influences the requirements needed to create the mappings. Studying political biases in the recommendation system,
% for example, requires mapping the videos to a partisan scale, whereas studying mainstream or popularity biases in the recommendation system
% requires mapping the videos to a popularity scale, which has more to do with the metadata of the videos rather than the actual content.

% We make use of existing works on evaluating Twitter users based on their similar interests \cite{twitter1, twitter2, twitter3}, in 
% order to develop a generic evaluation framework. If the hypothesis test relates to video content, we develop word/sentence embeddings representative 
% of that content. Embedding $A$ would represent the left-end of the scale and embedding $B$ would represent the right-end. Now, given a 
% query video $u$, we extract its word/sentence embeddings, and compute its cosine similarity score to both embeddings $A$ and $B$. 
% The difference between these two similarity scores gives us the scale mapping required to evaluate the content of the video, with respect to all previously seen videos, as well as to videos seen in the future.
% \dd{The exact formula with notation here may be helpful. -Daniyal}

% \para{Embedding creation.} We make use of Reddit in order to curate
% disparate set of embeddings based on different content, with methodologies used in previous works \cite{reddit1, reddit2, reddit3}. The exact subreddits considered are hypothesis dependent and we 
% will discuss them more in \cref{research-inferences}. The overall structure, however, is as follows:

% \begin{itemize}

% \item\parai{Curation.} We explore subreddits on the left-end and right-end of some content A. Given a subreddit, we have the options of either 
% collecting all user posts, and using them for our embedding vectors, or using all the links to articles posted. We chose the latter as user
% comments are less representative of the language used in YouTube videos, regardless of the left-right end of the scale. 
% Mapping videos related to political commentary, for example, should be evalauted using embeddings created through new articles, and not 
% on the comments made by the audience of the new articles. For more niche hypotheses, however, it may make more sense to create embeddings based on the general user language. 

% \item\parai{Vectorization.} Based on the textual features collected through the subreddits, we map them onto vectors using the 
% sentence embeddings model BERT \cite{bert}. We use BERT because it is fairly state-of-the-art in the realm of NLP, and, more 
% importantly, it does not require a secondary document for comparison, making it suited for our loose-classification task.

% \item\parai{Similarity computation.} The created BERT embeddings are now going to be out evaluation baselines. The similarity scores are 
% based on existing works \cite{twitter-score} Given a query video $u$, we
% compute its BERT vector and compute its cosine similarity to the left-end embedding $A$ and right-end embedding $B$. Our eventual 
% mapping will be computed by the following formula:
% $$ CMap(u) = S_{cos}(u,A) - S_{cos}(u,B) $$ 

% Given this mapping, a positive sign would indicate the content is similar to $A$, whereas a negative sign would indicate that the 
% content is similar to $B$. The magnitude would indicate the degree 
% of similarity to either $A$ or $B$. This mapping allows us to, very simply, map individual nodes to 1-D values that we may use for hypothesis testing, regardless of what hypothesis it is that we want to test. 

% \end{itemize}

% \subsection{Impact on research inferences}

% Given the impact variations in crawl parameters have on the resulting recommendation trees, we hypothesize that these differences
% permeate to differences in higher-level research inferences that researchers have made over the years. More specifically, given the above framework, 
% we will now test well studied YouTube bias studies, showing that the way the crawls are conducted impact the results we see in the 
% recommendations.

% \para{Hypothesis $h_{NvM}$: The niche vs mainstream bias hypothesis.} In order to validate this hypothesis, we need to show that the recommendation system
% can sway anywhere from niche content to mainstream content, based on the parameters altered during crawls. There is considerable work
% in the recommendation system space that concludes that there is either a polarizing bias or centrist bias \cite{idrama, rabbithole}. Instead of 
% getting into the breakdown of what qualifies as centrist/leftist/rightist, we make the test a little simpler, understanding whether the recommendation system pulls 
% users towards niche content or towards mainstream content. Determining
% the \emph{niche-ness} or \emph{mainstream-ness} of a channel requires some semantics, therefore we define niche content through the following:

% \para{Niche content is less popular than mainstream content.} Niche channels on YouTube have a smaller user base
% in comparison to mainstream channels. Niche videos comprise of fewer view counts and niche channels 
% comprise of fewer subscribers. We therefore consider all videos with under x views and channels with 
% fewer than y subscribers as niche videos/channels.

% \para{Niche content is homogenous.} Niche content tends to focus on singular topics, gaining a fan base 
% in that particular \emph{niche}. Mainstream content attempts to encompass a wide range of topics
% in order to gain a wider user base. We therefore identify channel topics and classify them in terms of the number unique topics that the channel covers. 

% The overall channel/video classification is, therefore, based on an intersection of these two paramterers.

% \subsubsection{The testing framework.} We collect a training set of videos gathered through the r/Conservative subreddit \cite{rconservative} and begin generating the recommendation trees through the seed {x}. The parameters altered for this test can be seen in Table \ref{table:nvm}.

% \subsubsection{Evaluation.} Based on the niche/mainstream classification, we identify develop labels for the 
% values in each of the nodes, with some scalar in order to understand the intensity.

% \para{Hypothesis $h_{s}$: The unsafe kids content hypothesis.} In order to validate this hypothesis, we
% need to show that the recommendation system can be pruned in a way that the recommendations seen could be safe or unsafe, with no conclusive `bias'. The training set comprises of videos gathered from the 
% r/KidSafeVideos subreddit, and the seed is x.

% \subsubsection{The testing framework.} During the tree generation phase, we routinely take screenshots of the videos playing 
% so that we may generate labels for the frame played in the video. We then leverage the Google Vision API \cite{google-vision} for screenshot annotation
% and then see if there were any suggestive, violent or inappropriate labels for any of the content played. 
% We also annotate the caption tracks, in order to identify any inappropriate language used in the videos.
% Given this annotation, we can then label nodes as either safe/unsafe along with a scalar to understand the 
% intensity of the \emph{(un)safe-ness}. An intersection of the visual and textual labels helps us reduce 
% the videos to a set of labels for reductive analysis.

% \subsubsection{Evaluation.}

% \para{Hypothesis $h_{md}$: The metadata bias hypothesis.} 









==> tex-files/train-results.tex <==
\section{Channel diversity and popularity results} \label{sec:train-seed-results}

In this section we will analyse the resulting variations of the trees on two levels: (1) the intra-tree variations that are merely a result of the
nodes' \emph{position} in the respective trees, and (2) the inter-tree variations that are a result of the (training set, seed) pairs. We will analyse
these differences in terms of the channel entropies and recommended videos' popularities. Each node is considered to be the set of all videos 
recommended to the user as some level $i$ and depth $k$. Our goal is to show that given these recommendation set trees: (a) there is a noticeable 
difference in means of the distributions and (b) this difference is statistically significant across all trees/positions.

\subsection{Popularity}

\begin{figure}[t]
  \centering
  \includegraphics[width=.45\textwidth]{plots/kde-views.pdf}
  \caption{Log scaled tree views collapsed together by tuple type.
  % Traversing a path in this tree involves watching the video associated with
  % a node and adding child nodes which represent the subsequent
  % recommendations.
  }
  \label{fig:results:tuple-views}
\end{figure}


\subsubsection{Tuple selection.} 

\Cref{fig:results:tuple-views} shows the view count variations that are the result of tuple type. When considering
the mean views of the tuples, we see the following:

\parai{Seed selection has a biggest impact on the resulting recommendations' views.}i th simply changing the seed from niche to mainstream results in nearly twice the number of the views when compared
to the like training set. Furthermore, regardless of the training set, the views change by at least $~800,000$. The KS-test also showed that
there are statistically significant variations between \emph{all the tuple pairs}. This means that selection of both tuple entry types result in significantly
varying view counts of the resulting recommendations. We see that by simply picking a seed that is either 
niche/mainstream, regardless of all previous training, heavily skews the popularity of the
resulting recommendations. Mainstream seeds always result in higher views than niche seeds and, while the training set has \emph{some} impact on 
the recommendations' popularity, it is not enough to offset the direct impact the seeded video has on the resulting views. Simply switching the
seed from niche to mainstream, despite a mainstream training set in both cases, results with an increased mean of 1.88M views, thus signifying the
magnitude seed selection has.

\parai{Training set differences are also statistically significant.} While changing the training set and keeping the seed constant does
not create as much of a difference as changing the seed does, the results are still statistically significant, thus showing that training set 
selection does have a significant impact of the resulting recommendations, albeit by a smaller magnitude. 

\para{Impact on research inferences.} Given these results, we conclude that researchers must pay particular attention to profile training,
as profiles not trained sufficiently will be heavily biased given the seed video. We also conclude that, despite the niche training set containing
videos with < 5000 views, the resulting recommendations still gained over a million views. This shows that regardless of
the seed or training set, the recommendation system has an implicit popularity bias.

\begin{figure}[t]
  \centering
  \includegraphics[width=.45\textwidth]{plots/kde-position-views.pdf}
  \caption{Log scaled path views collapsed together by their relative positions in the trees.
  % Traversing a path in this tree involves watching the video associated with
  % a node and adding child nodes which represent the subsequent
  % recommendations.
  }
  \label{fig:results:tuple-position-views}
\end{figure}

\subsubsection{Node position.} 

\Cref{fig:results:tuple-position-views} shows the impact position on the trees have on the resulting views of the 
recommendations. Taking position into consideration, we see some clear patterns:

\parai{Videos seen at the start are more popular than videos seen towards the end.} The figure shows that the top of the tree has, on average, 2.33M
more views than the leaf nodes, showing that the initial videos recommended by the algorithm are much more popular than the videos recommended
after users have been viewing content for a while. The KS-test also shows that there is a statistically significant difference in the views seen at the 
start of the crawls, versus at the end of the crawls, thus signifying an initial popularity bias.

\parai{Videos at the right of the tree are more popular than videos at the left of the tree.} The left-most path consists of the top recommended videos 
of the entire tree whereas the right-most path consists of videos at the very bottom of the recommendation tree. The figure shows that the right-most 
path of the tree contains recommended videos with 0.76M more views than the videos recommended in the left. The KS-test also shows a statistically 
significant difference between the two paths, highlighting the popularity bias towards the lower end of the recommendation tab.

\para{Impact on research inferences.} Given these results, we conclude that simply traversing a recommendation chain is insufficient in concluding the
completeness of the recommendation tree. Node position and edge direction has a direct impact on the popularity of the resulting recommendations, 
therefore, bias studies leveraging random-walks or single-path traversals lack the completeness necessary to make accurate claims on the 
popularity bias in the recommendation system.

\subsection{Channel diversity}

\begin{figure}[t]
  \centering
  \includegraphics[width=.45\textwidth]{plots/kde-entropy.pdf}
  \caption{Channel entropies with trees collapsed together by tuple type.
  % Traversing a path in this tree involves watching the video associated with
  % a node and adding child nodes which represent the subsequent
  % recommendations.
  }
  \label{fig:results:kde-entropy}
\end{figure}

\subsubsection{Tuple selection.} \Cref{fig:results:kde-entropy} shows the channel entropies distributed across trees given all the tuple pairs. 
Given these relative entropies, we see:

\parai{Niche seeds always result in higher entropies.} Regardless of training set type, the recommended channel entropies are always higher when the 
seeds are niche. While one may assume that this would also translate to the (\Tniche, \Smain) > (\Tmain, \Smain), our results show the opposite. This 
shows that despite the niche seed creating a significant difference in skewing the diversity of the recommended channels, the training set signal
to the recommendation system is not significant enough to warrant more diverse content.

\parai{The KS-test results are statistically significant only when the seed changes.} All statistical significance tests result in $p$-values $< 0.05$
only when the seeds in the tested tuples are flipped. This shows that there is no impact of the training set in the diversity of the recommended content.

\para{Impact on research inferences.} Our tests show that diverse content is contingent on seed alone, therefore works aiming to identify possible 
fringe communities or radical bubbles must pay particular attention to the seed chosen. Secondly, we consistently see the channel diversity to be
notably \emph{higher} whenever the recommendation system picks up on niche signals. This implies that systems aiming to find an echo-chamber/fringe 
community bias will actually conclude the opposite, while certain paths may get users to some extreme, the recommendation system is, hollistically, 
geared towards introducing additional options to users possibly trying to \emph{go down some rabbit-hole.} The recommendation system does not 
introduce these options when users are engaging with mainstream content, thus showing an inherit bias to pull users away from possible
niche extremes.

\begin{figure}[t]
  \centering
  \includegraphics[width=.45\textwidth]{plots/kde-position-entropy.pdf}
  \caption{Channel entropies with paths collapsed together by their relative positions in the trees.
  % Traversing a path in this tree involves watching the video associated with
  % a node and adding child nodes which represent the subsequent
  % recommendations.
  }
  \label{fig:results:kde-position-entropy}
\end{figure}

\subsubsection{Node position.}

\Cref{fig:results:kde-position-entropy} shows the channel entropies distributed along various positions on the trees. The KS-test on the left-most
and right-most paths result in a statistically significant difference, thus showing that recommended channels appearing later in the recommendations
tab have a tendency to be more diverse. 











